Adams' cobar construction as a monoidal $E_{\infty}$-coalgebra model of the based loop space

We prove that the classical map comparing Adams' cobar construction on the singular chains of a pointed space and the singular cubical chains on its based loop space is a quasi-isomorphism preserving explicitly defined monoidal $E_\infty$-coalgebra structures. This contribution extends to its ultimate conclusion a result of Baues, stating that Adams' map preserves monoidal coalgebra structures.

==> aux/immersion.tex <==
\boxed{\begin{tikzpicture}[scale=.6]
\draw (1,3.7) to (1,3); 

\draw (1,3) to [out=205, in=90] (0,0);

\draw [shorten >= 0cm] (.6,2.73) to [out=-100, in=90] (2,0);

\draw [shorten >= .15cm] (1,3) to [out=-25, in=30, distance=1.1cm] (1,1.5);
\draw [shorten <= .1cm] (1,1.5) to [out=210, in=20] (0,1);

\node at (1,3.9){};
\node at (0,-.32){};
\node at (2,-.32){};

\node at (3,1.5){$\sim$\ \ \ };
\end{tikzpicture}
\begin{tikzpicture}[scale=.6]
\draw (1,3.7) to (1,3); 

\draw [->](1,3) to [out=205, in=90] (0,0);

\draw [shorten >= 0cm,->] (.6,2.73) to [out=-100, in=90] (2,0);

\draw [shorten >= .15cm] (1,3) to [out=-25, in=30, distance=1.1cm] (1,1.5);
\draw [shorten <= .1cm] (1,1.5) to [out=210, in=20] (0,1);


\def\x{.8}

\node[scale=\x] at (1,3.9){$\scriptstyle 1$};

\node[scale=\x] at (.7,3.05){$\scriptstyle 1$};
\node[scale=\x] at (1.35,3.05){$\scriptstyle 2$};

\node[scale=\x] at (.1,2.3){$\scriptstyle 1$};
\node[scale=\x] at (.8,2.3){$\scriptstyle 2$};

\node[scale=\x] at (-.15,1.3){$\scriptstyle 1$};
\node[scale=\x] at (.3,1.3){$\scriptstyle 2$};

\node[scale=\x] at (0,-.3){$\scriptstyle 1$};
\node[scale=\x] at (2,-.3){$\scriptstyle 2$};
\end{tikzpicture}}

==> aux/relations.tex <==
\begin{equation*}
\boxed{\begin{tikzpicture}[scale=.28]
\draw (-4,0)--(-4,2)--(-5,3)--(-5,4);
\draw (-6,0)--(-6,2)--(-5,3)--(-5,4);
\node [scale=.8] at (-4.2,3.2) {$\Delta$};
\draw [fill] (-6,.2) circle [radius=.2];
\node [left] at (-6,0) {$\varepsilon$};

\node at (-2,2) {=};
\draw (0,0)--(0,4);
\node at (2,2) {=};

\draw (4,0)--(4,2)--(5,3)--(5,4);
\draw (6,0)--(6,2)--(5,3)--(5,4);
\node [scale=.8] at (4.2,3.2) {$\Delta$};
\draw [fill] (6,.2) circle [radius=.2];
\node [right] at (6,0) {$\varepsilon$};
\end{tikzpicture}
\qquad \qquad
\begin{tikzpicture}[scale=.28]
\node at (0,2){=};
\node at (0,0) {\phantom{$\varepsilon$}};

\draw (2,0)--(3,1)--(3,2)--(4,3)--(4,4);
\draw (4,0)--(3,1);
\draw (4,3)--(5,2)--(5,0);
\node [scale=.8] at (3.2,3.2) {$\Delta$};
\node [scale=.8] at (2.2,1.2) {$\Delta$};

\draw (-2,0)--(-3,1)--(-3,2)--(-4,3)--(-4,4);
\draw (-4,0)--(-3,1);
\draw (-4,3)--(-5,2)--(-5,0);
\node [scale=.8] at (-3.2,3.2) {$\Delta$};
\node [scale=.8] at (-2.2,1.2) {$\Delta$};

\node at (5.3,0){};
\end{tikzpicture}}
\end{equation*}

==> aux/surjection_like.tex <==
\begin{equation*}
\begin{tikzpicture}[scale=1]
\draw (0,0)--(0,-.6) node[below, scale=.75]{$1$};
\draw (0,0)--(.5,.5);
\draw (-.3, .3)-- (-.2,.5) node[scale=.75] at (-.2,.7) {\qquad $1\, \ \ 2\ \ ...\ \ k_1$};
\draw (-.5,.5)--(0,0);
\node[scale=.75] at (.11,.4){$..$.};

\node[scale=.75] at (1,0){$\cdots$};
\node[scale=.75] at (1,-.9){$\cdots$};

\draw (2,0)--(2,-.68) node[scale=.75, below]{$r$};
\draw (2,0)--(2.5,.5);
\draw (1.7, .3)--(1.8,.5) node[scale=.75] at (1.78,.7) {\qquad $1\, \ \ 2\ \ ...\ \ k_r$};
\draw (1.5,.5)--(2,0);
\node[scale=.75] at (2.11,.4){$..$.};

\draw (1,2.5)--(1,3) node[scale=.75, above]{$1$};
\draw (1,2.5)--(0,2) node[scale=.75, below]{$1$};
\draw (.25,2.125)--(.5,2) node[scale=.75, below]{$2$};
\draw (.5,2.25)--(1,2) node[scale=.75, below]{$3$};
\draw (1,2.5)--(2,2) node[scale=.75, below]{\ \quad $n + r$};
\node[scale=.75] at (1.5,1.75){$\cdots$};

\node[scale=.75] at (1,1.3) {$\vdots$};

\node at (2.85,0){};
\end{tikzpicture}
\end{equation*}

==> sec/categorical.tex <==
% !TEX root = ../cobar1.tex

\section{Cubical cobar construction}

We construct a cubical model for the based loop space using necklical sets, a notion related to both simplicial sets and cubical sets.
Similar constructions and results may be found in \cite{baues1980geometry}, \cite{berger1995loops}, \cite{baues1998hopf}, \cite{dugger2011rigidification}, \cite{galvez2020hopf}, and \cite{rivera2018cubical, rivera2019path}.

\subsection{Necklical sets}

Let us consider the subcategory $\simplex_{*,*}$ of the simplex category $\simplex$ with the same objects and morphisms given by functors $f \colon [n] \to [m]$ satisfying $f(0) = 0$ and $f(n) = m$.
It is a strict monoidal category when equipped with the monoidal structure $[n] \ot [m] = [n+m]$, thought of as identifying the elements $n \in [n]$ and $0 \in [m]$, and unit given by $[0]$.
In passing, we mention that this category is $\op$-dual to the augmented simplex category, a form of Joyal duality.

The \textit{necklace category} $\Nec$ is obtained from $\simplex_{*,*}$ as follows.
Thinking of $\simplex_{*,*}$ as a monoid in $\Cat$, we first apply the bar construction to it and produce a simplicial object in $\Mon_{\Cat}$ which, after realization, defines the strict monoidal category $\Nec$.
We denote the monoidal structure by
\[
\vee \colon \Nec \times \Nec \to \Nec.
\]
We describe $(\Nec, \vee)$ in more explicit terms.
The objects of $\Nec$, called \textit{necklaces}, are freely generated by the objects of $\simplex_{*,*}$ through the monoidal structure $\vee$.
Namely, the set of objects of $\Nec$ is given by
\[
\big\{ [n_1] \vee \dots \vee[n_k] \mid n_i, k \in \N_{>0} \big\}
\]
together with $[0]$ serving as the monoidal unit.

The morphisms of $\Nec$ are generated through the monoidal structure by the following four types of morphisms:
\begin{enumerate}
	\item $\partial^j \colon [n-1] \to [n]$ for $j = 1, \dots, n-1$,
	\item $\Delta_{[j], [n-j]} \colon [j] \vee [n-j] \to [n]$ for $j = 1, \dots, n-1$,
	\item $s^j \colon [n+1] \to [n]$ for $j = 0, \dots, n$ and $n>0$, and
	\item $s^0 \colon [1] \to [0]$.
\end{enumerate}
We may identify $\Nec$ with a full sub-category of the category of double pointed simplicial sets $\sSet_{*,*}$ as follows.
Consider the functor
\[
\mathcal{S} \colon \Nec \to \sSet_{*,*}
\]
induced by sending any necklace $T = [n_1] \vee \dots \vee[n_k]$ to the simplicial set
\[
\mathcal{S}(T) = \simplex^{n_1} \vee \dots \vee \simplex^{n_k},
\]
where the wedge symbol now means we identify the last vertex of $\simplex^{n_i}$ with the first vertex of $\simplex^{n_{i+1}}$ for $i = 1, \dots, k-1$ and the two base points are given by the first vertex of $\simplex^{n_1}$ and the last vertex of $\simplex^{n_k}$.
Then $\mathcal{S}$ is a fully faithful functor, so $\Nec$ may be identified with the full sub-category of $\sSet_{*,*}$ having as objects those double pointed simplicial sets of the form $\simplex^{n_1} \vee \dots \vee \simplex^{n_k}$.
The \textit{dimension} of a necklace $T = [n_1] \vee \dots \vee[n_k]$ is defined by $\dim(T) = n_1 + \dots + n_k-k$.

The (non-symmetric) monoidal category of \textit{necklical sets} $\Fun(\Nec^{\op}, \Set)$ equipped with Day convolution (\cref{ss:day convolution}) is denoted by $\nSet$.

\subsection{From necklaces to cubes}

We now describe a categorical version of Adams' maps $\theta_n \colon \gcube^{n-1} \to P(\gsimplex^{n};0,n)$ by constructing a monoidal functor
\[
\cP \colon \Nec \to \cube.
\]

We first set $\cP([0])=2^0$.
On any other necklace $T \in \Nec$ we define $\cP(T) = 2^{\dim(T)}$.
In order to define $\cP$ on morphisms, it is sufficient to consider the following cases.
\begin{enumerate}
	\item For any $\partial^j \colon [n] \to [n+1]$ such that $0< j<{n+1}$, define $\cP(\partial^j) \colon 2^{n-1}\to 2^{n}$ to be the cubical coface functor $\cP(f)= \delta_0^{j}$.

	\item For any $\Delta_{[j], [n+1-j]} \colon [j] \vee [n+1-j] \to [n+1]$ such that $0<j<n+1$, define
	\[
	\cP(\Delta_{[j], [n+1-j]}) \colon 2^{n-1}\to 2^{n}
	\]
	to be the cubical coface functor $\cP(f)=\delta_1^{j}$.

	\item We now consider morphisms of the form $s^j \colon [n+1] \to [n]$ for $n>0$.
	If $j=0$ or $j=n$, then $\cP(f) \colon 2^n \to 2^{n-1}$ is defined to be the cubical codegeneracy functor $\cP(s^j)= \varepsilon^{j}$.
	If $0<j<n$, then we define $\cP(s^j) \colon 2^n \to 2^{n-1}$ to be the cubical coconnection functor $\gamma^{j}$.

	\item For $s^0 \colon [1] \to [0]$ we define $\cP(s^0) \colon 2^0 \to 2^0$ to be the identity functor.
\end{enumerate}

\begin{remark}
	The functor $\cP$ is neither faithful or full.
	However, for any necklace $T' \in \Nec$ with $\dim(T')=n+1$ and any cubical coface functor $\delta_{\epsilon}^j \colon 2^n \to 2^{n+1}$ for $0 \leq j \leq n+1$, there exists a unique pair $(T, f \colon T \hookrightarrow T')$, where $T \in \Nec$ with $\dim(T)=n$ and $f \colon T \hookrightarrow T'$ is an injective morphism in $\Nec$, such that $\cP(f) = \delta_{\epsilon}^j$.
	\todo{@manuel:Why the pair? It seems that the map has all the information.}
\end{remark}

The functor $\cP \colon \Nec \to \cube$ induces an adjunction between $\cSet$ and $\nSet$ with right and left adjoint functors given respectively by
\[
\cP^\ast \colon \cSet \to \nSet,
\qquad \text{and} \qquad
\cP_{!} \colon \nSet \to \cSet.
\]
Explicitly, for a cubical set $Y \colon \cube^\op \to \Set$,
\[
\cP^\ast(Y)= Y \circ \cP^\op,
\]
and for a necklical set $K \colon \Nec^\op \to \Set$,
\[
\cP_{!}(K) \ =
\colim_{\mathcal{Y}(T) \to K} \cP(T) \ \cong
\colim_{\mathcal{Y}(T) \to K} \cube^{\dim(T)}.
\]
Since $\cP$ is a monoidal functor, the functor $\cP_{!} \colon \nSet \to \cSet$ is a monoidal as well.

\subsection{Cubical cobar construction}\label{ss:cubical cobar}

Using the framework of necklical sets, we may reinterpret a Baues' geometric cobar construction from \cite{baues1998hopf} as a functor
\[
\ncobar \colon \sSet^0 \to \Mon_{\nSet},
\]
which we now define.

For any reduced simplicial set $X$, we define a necklical set $\ncobar(X) \colon \Nec^\op \to \Set$ having as necklical cells all necklaces inside $X$; namely
\[
\ncobar(X) \, = \! \colim_{\mathcal{S}(T) \to X} \mathcal{Y}(T).
\]
The monoidal structure $\vee \colon \Nec \times \Nec \to \Nec$ given by concatenation of necklaces induces a natural product
\[
\ncobar(X) \ot \ncobar(X) \to \ncobar(X)
\]
making $\ncobar(X)$ into a monoid in the monoidal category $\nSet$.

We may now define the \textit{cubical cobar construction}
\[
\ccobar \colon \sSet^0 \to \Mon_{\cSet}
\]
as the composition
\[
\ccobar = \cP_! \, \ncobar.
\]
This reinterpretation of Baues construction in terms of cubical sets was also studied in \cite{rivera2018cubical}.

\subsection{Relation to the cobar construction}

We now relate the cubical cobar functor $\ccobar \colon \sSet^0 \to \Mon_{\cSet}$ to the cobar construction $\cobar \colon \coAlg \to \Mon_{\Ch}$ (\cref{ss:cobar construction}).

\begin{theorem}\label{t:ccobar and cobar}
	There is a natural isomorphisms of functors
	\[
	\cchains \ccobar \cong \cobar \schainsA \colon \sSet^0 \to \Mon_{\Ch}.
	\]
\end{theorem}

\begin{proof}
	Denote by $\iota_n \in (\cube^n)_n$ the top dimensional non-degenerate element of the standard $n$-cube $\cube^n$.
	Note that for a reduced simplicial set $X$, we may represent any non-degenerate $n$-cube $\alpha \in (\cP_!(\ncobar(X)))_n$ as a pair $\alpha = [\sigma \colon \mathcal{Y}(T) \to X, \iota_n]$ for some $T = [n_1] \vee \dots \vee [n_k] \in \Nec$ with $\dim(T) = n_1 + \dots + n_k - k = n$.

	To define an algebra map
	\[
	\varphi_X \colon \cchains(\cP_!(\ncobar(X))) \xra{\cong} \cobar \schainsA(X)
	\]
	it suffices to define it on any generator of the form $\alpha=[\sigma \colon \simplex^{n+1} \to X, \iota_{n}]$, i.e., when $T$ is of the form $T = [n+1]$, for some $n \geq 0$.
	If $n = 0$ let $\varphi_X(\alpha)= [\overline{\sigma}] + 1_\k$, where $[\overline{\sigma}] \in s^{-1} \overline{ \schains(X)} \subset \cobar \schainsA(X)$ denotes the (length $1$) generator in the cobar construction of $\schains(X)$ determined by $\sigma \in X_{n+1}$ and $1_\k$ denotes the unit of the underlying ring $\k$.
	If $n > 0$, we let $\varphi_X(\alpha)=[\overline{\sigma}]$.
	A straightforward computation yields that this gives rise to a well defined isomorphism of algebras, which is compatible with the differentials, and natural with respect to maps of simplicial sets.
\end{proof}

A similar result to \cref{t:ccobar and cobar} was observed in the case of $1$-reduced simplicial sets in \cite[Section~3.5]{berger1995loops}.

\subsection{A monoidal coalgebra structure on the cobar construction}

TBW

==> sec/monoidal.tex <==
% !TEX root = ../cobar1.tex

\section{Monoidal properties of \texorpdfstring{$\UM$}{UM}-coalgebras} \label{s:monoidal}

The first goal of this section is to construct a monoidal structure on $\coAlg_\UM$.
We will do so by providing $\M$ with the structure of a Hopf prop.
Then, we will show that the functor $\cchainsUM \colon \cSet \to \coAlg_{\UM}$ defined in \cref{ss:e-infty on cubical} is monoidal.

\subsection{Monoidal structures on presheaves} \label{ss:day convolution}

Let $\sA$ be a small category and $P$ and $P^\prime$ two presheaves over $\sA$.
Their \textit{Cartesian product} is defined by
\[
(P \times P^\prime)(a) = P(a) \times P^\prime(a),
\]
and, if $(\sA, \otimes)$ is a monoidal category, their \textit{Day convolution product} by
\[
P \otimes P^\prime \, = \! \colim_{\substack{\yoneda(a) \to P \\ \yoneda(a^\prime) \to P^\prime}} \yoneda(a \otimes a^\prime).
\]
These constructions induce natural monoidal structures on the category of presheaves over $\sA$.

We will consider $\sSet$ with the Cartesian product and $\cSet$ with Day convolution.

\subsection{Triangulation and its right adjoint} \label{ss:triangulation and its adjoint}

As we recall below, simplicial and cubical sets can be related using the simplicial cubes $(\simplex^1)^{\times n}$, which define a functor $\cube \to \sSet$.

The \textit{triangulation} functor $\triangulate \colon \cSet \to \sSet$ is the Yoneda extension of this functor.
Explicitly,
\[
\triangulate(Y) = \colim_{\cube^n \to Y} (\simplex^1)^{\times n}.
\]
It has a right adjoint $\mathcal{U} \colon \sSet \to \cSet$ which is given by the formula
\[
\mathcal{U}(X)_n = \sSet \big( (\simplex^1)^{\times n}, X \big).
\]

With the monoidal structure defined in \cref{ss:day convolution}, the triangulation functor is monoidal.
Thus, it induces a functor
\[
\triangulate \colon \Mon_{\cSet} \to \Mon_{\sSet}
\]
between the associated categories of monoids.

\subsection{Serre coalgebra} \label{ss:serre coalgebra sym monoidal}

Recall that both $\Ch$ and $\coAlg$ are symmetric monoidal categories.
If $\cSet$ is equipped with the Day convolution monoidal structure (\cref{ss:day convolution}), then the functors $\cchains$ and its lift $\cchainsA$ are monoidal.
Together with straightforward computations, these statements follow from the fact that the chain complexes $\chains(\cube^p) \otimes \chains(\cube^q)$ and $\chains(\cube^{p+q})$ are canonically isomorphic for any $p, q \geq 0$.

For later reference we record the following consequence of the previous claims and the fact that, for any coalgebra, the braiding $x \otimes y \mapsto (-1)^{\bars{x} \bars{y}} y \otimes x$ is a morphism of coalgebras.

\begin{lemma} \label{l:serre diagonal invariant}
	Let $\sigma \in \S_d$ acting on $\chains(\cube^1)^{\otimes d}$ by permuting tensor factors, then
	\[
	\begin{tikzcd}
		\chains(\cube^1)^{\otimes d} \arrow[r, "\Delta"] \arrow[d, "\sigma"] &
		\chains(\cube^1)^{\otimes d} \otimes \chains(\cube^1)^{\otimes d} \arrow[d, "\sigma \otimes \sigma"] \\
		\chains(\cube^1)^{\otimes d} \arrow[r, "\Delta"] &
		\chains(\cube^1)^{\otimes d} \otimes \chains(\cube^1)^{\otimes d}
	\end{tikzcd}
	\]
	commutes.
\end{lemma}

\subsection{Alexander--Whitney coalgebra}

The functors of simplicial chains $\schains$ and its lift $\schainsA$ to $\coAlg$ (\cref{ss:aw coalgebra}) are not monoidal in the strict sense.
Nonetheless, with the Eilenberg--Zilber map $\schains(X) \otimes \schains(Y) \to \schains(X \times Y)$ they are lax monoidal functors, a sufficient condition for monoids to be sent to monoids.

\subsection{Hopf operads and \pdfEinfty-bialgebras}

So far we have consider operad and props over the category $\Ch$ but, since $\coAlg$ is also a symmetric monoidal category, we can consider them over $\coAlg$.
That is to say, demand that all defining chain complexes be coalgebras and all compositions be morphisms of these.
We refer to operads and props over $\coAlg$ as \textit{Hopf operads and props} respectively.

If $\cO$ is a Hopf operad, the category $\coAlg_\cO$ is monoidal.
The structure maps of a product of $\cO$-coalgebras $C \otimes C^\prime$ are given by
\[
\begin{tikzcd} [column sep = normal, row sep=normal]
	\cO(r) \otimes (C \otimes C^\prime) \arrow[r, "\Delta_\cO \otimes \id"] &[10 pt] \cO(r) \otimes \cO(r) \otimes (C \otimes C^\prime) \arrow[d, "Sh"'] &[-0pt] \\ &
	\big(\cO(r) \otimes C \big) \otimes \big( \cO(r) \otimes C \big) \arrow[r] &
	C^{\otimes r} \otimes C^{\prime\, \otimes r} \arrow[d, "Sh"] \\
	& & (C \otimes C^\prime)^{\otimes r}.
\end{tikzcd}
\]
If $\cO$ is a Hopf $E_\infty$-operad we refer to monoids in $\coAlg_\cO$ as $E_\infty$-\textit{bialgebras}.

Similarly, if $\cP$ is a Hopf prop then its category of representations is also monoidal.

\subsection{Cubical structure on $\M$}

We will now revisit from \cref{ss:definition of M} the definition of $\M$ and provide this prop with a cubical structure.
We will use this in \cref{ss:hopf prop M} to provide $\M$ with the structure of a Hopf prop.

We start with a general observation.
As explained in \cref{ss:free constructions}, the $(m,n)$-part of the free prop generated by an $\S$-module $N$ is given by
\[
\free(N)(m,n) \ = \bigoplus_{\Gamma \in \graphs(m,n)} \bigotimes_{v \in Vert(\Gamma)} out(v) \otimes_{\S_q} N(p, q) \otimes_{\S_p} in(v),
\]
which is well defined only up to a choice of total order on the set of vertices of the $(m,n)$-graphs involved.

In the case we are concern with, the free prop whose quotient defines $\M$ is generated by the $\S$-bimodule $M$ with:
\[
M(1,0) = \k \Big\{ \; \raisebox{-3pt}{\counit} \ \Big\}, \qquad
M(1,2) = \k[\S_2] \Big\{ \, \raisebox{-2.5pt}{\coproduct} \hspace*{2pt} \Big\},
\]
\[
M(2,1) =
\k[\S_2^\op] \Big\{ \partial_0 \raisebox{-2.5pt}{\product} \hspace*{1pt} \Big\} \xleftarrow{1 - T}
\k[\S_2^\op] \Big\{ \, \raisebox{-2.5pt}{\product} \hspace*{2pt} \Big\},
\]
and $M(m,n) = 0$ otherwise.
We notice that the elements $\rightboundary\,$ and $\,\leftboundary\,$ in $\free(M)(2,1)$ are interchanged by the action of $T \in \S_2^\op$.
Let $\widetilde{\M}$ be the quotient of $\free(M)$ by the ideal generated by the identification of $\,\partial_0 \raisebox{-1.5pt}{\product}$ and $\,\rightboundary\,$, so that the boundary of $\product$ is $\,\boundary\,$.
Consider a basis element of $\widetilde{\M}(m,n)_d$ represented by an immersed $(m,n)$-graph $\Gamma$ with $d$ occurrences of $\product$.
A choice of total order of the vertices of $\Gamma$ defines a chain map
\begin{equation} \label{e:order chain map}
	\begin{tikzcd}[row sep=0, column sep=small]
		\iota_\Gamma \colon \chains(\cube^d) \arrow[r] & \widetilde{\M}(m,n) \\
		\qquad {[0,1]}^{\otimes d} \arrow[r, |->] & \Gamma,
	\end{tikzcd}
\end{equation}
referred to as the \textit{characteristic map of $\Gamma$}.
We obtain characteristic maps on $\M$ simply by composing these with the projection $\widetilde{\M} \to \M$ induced from the quotient by the prop ideal generated by the relations \eqref{e:relations of M}.

\subsection{Hopf structure on $\M$} \label{ss:hopf prop M}

We now use the existence of characteristic maps on $\M$ to show it is a prop over $\coAlg$.
We will show the following is well defined in \cref{t:cubical structure on M}.

\begin{definition}
	The \textit{coproduct} $\Delta_\M \colon \M \to \M^{\otimes 2}$ is defined on basis elements $\Gamma$ by
	\[
	\Delta_{\M}(\Gamma) = \iota_\Gamma^{\otimes 2} \circ \Delta \left( [0,1]^{\otimes d} \right),
	\]
	where $d = \bars{\Gamma}$, and the \textit{counit} $\epsilon_\M \colon \M \to \underline{\k}$ by requiring $\epsilon_M(\Gamma) = 1$ if the degree of $\Gamma$ is $0$, where $\underline{\k}$ is the $\S$-bimodule with $\underline{\k}(m,n) = \k$.
\end{definition}

We remark that this coalgebra structure is obtained by extending monoidally to directed graphs the assignments:
\begin{align*}
	&\Delta_\M && \varepsilon_\M \\
	\coproduct & \mapsto \coproduct \otimes \coproduct \,, &
	\coproduct & \mapsto 1, \\
	\counit \ & \mapsto \ \counit \ \otimes \ \counit \,, &
	\counit \ & \mapsto 1, \\
	\product & \mapsto \rightboundary \ \otimes \product + \product \otimes \ \leftboundary \,, &
	\coproduct & \mapsto 0.
\end{align*}

\begin{theorem} \label{t:cubical structure on M}
	The maps $\Delta_\M$ and $\varepsilon_\M$ are well defined and make $\M$ into a Hopf prop.
\end{theorem}

\begin{proof}
	By \cref{l:serre diagonal invariant} these maps are independent of the total order on vertices used to define characteristic maps.

	The linear map $\Delta_\M$ is compatible with the relations defining $\M$ since
	\begin{center}
		\hspace*{2cm}
		\begin{tikzcd}
			\leftcounitcoproduct \arrow[r, "\Delta_\M"] \arrow[d, <->] &[-0pt] \leftcounitcoproduct \otimes \leftcounitcoproduct \arrow[d, <->] \\
			\identity \arrow[r, "\Delta_\M"] & \ \, \identity \otimes \identity \, ,
		\end{tikzcd}
		\hfill
		\begin{tikzcd}
			\rightcounitcoproduct \arrow[r, "\Delta_\M"] \arrow[d, <->] &[-0pt] \rightcounitcoproduct \otimes \rightcounitcoproduct \arrow[d, <->] \\
			\identity \arrow[r, "\Delta_\M"] & \ \, \identity \otimes \identity \, ,
		\end{tikzcd}
		\hspace*{2cm}
	\end{center}
	\begin{center}
		\hspace*{2cm}
		\begin{tikzcd}
			\leftcomb \arrow[r, "\Delta_\M"] \arrow[d, <->] &[-0pt] \leftcomb \, \otimes \leftcomb \arrow[d, <->] \\
			\rightcomb \arrow[r, "\Delta_\M"] & \, \rightcomb \, \otimes \rightcomb,
		\end{tikzcd}
		\hfill
		\begin{tikzcd}
			\productcounit \arrow[r, "\Delta_\M"] \arrow[d, <->] &[-0pt] \counit\ \counit \, \otimes \productcounit + \productcounit \otimes \, \counit\ \counit \arrow[d, <->] \\
			0 \arrow[r, "\Delta_\M"] & \ 0.
		\end{tikzcd}
		\hspace*{.6cm}
	\end{center}
	It is a chain map since
	\begin{center}
		\qquad
		\begin{tikzcd}
			\counit \arrow[r, "\Delta_\M"] \arrow[d, "\partial"'] &[-0pt] \counit \otimes \counit \arrow[d, "\partial"'] \\
			0 \arrow[r, "\Delta_\M"] & \ \, 0 \, ,
		\end{tikzcd}
		\hfill
		\begin{tikzcd}
			\coproduct \arrow[r, "\Delta_\M"] \arrow[d, "\partial"'] &[-0pt] \coproduct \otimes \coproduct \arrow[d, "\partial"'] \\
			0 \arrow[r, "\Delta_\M"] & \ \, 0 \, ,
		\end{tikzcd}
		\hfill
		\begin{tikzcd}
			\product \arrow[r, "\Delta_\M"] \arrow[d, "\partial"'] &[-0pt] \leftboundary \ \otimes \product + \product \otimes\ \rightboundary \arrow[d, "\partial"'] \\
			\rightboundary \,-\, \leftboundary \arrow[r, "\Delta_\M"] &
			\, \rightboundary \otimes \rightboundary \,-\, \leftboundary \otimes \leftboundary\,.
		\end{tikzcd}
	\end{center}
	One can check similarly that $\varepsilon_\M$ is a well defined morphism of $\S$-bimodules.

	Since we are using the Serre coalgebra structure, for each biarity $(m,n)$ we obtain a coalgebra.
	Furthermore, $\Delta_\M$ is compatible with the composition structure since for any pair of characteristic maps $\iota_\Gamma$ and $\iota_{\Gamma^\prime}$, the chain map $\iota_\Gamma \otimes \iota_{\Gamma^\prime}$ is a characteristic map for any composition of $\Gamma$ and $\Gamma^\prime$ with the induced order on vertices.
	The compatibility of $\epsilon_\M$ is immediate.
\end{proof}

\subsection{Monoidal \pdfEinfty-structures}

We now prove the main technical result of this paper.

\begin{lemma} \label{l:cubical e-infty chains are monoidal}
	The functor $\cchainsUM \colon \cSet \to \coAlg_\UM$ is monoidal.
\end{lemma}

\begin{proof}
	It suffices to prove this result for chains on the standard cubes.
	These are equipped with a natural $\M$-structure, and we will prove the stronger statement that the functor $\mathrm{N}^\cube_\M \colon \cube \to \biAlg_{\M}$ is monoidal.

	From \cref{ss:serre coalgebra sym monoidal} we know that the Serre diagonal and the augmentation map are compatible with the monoidal structure on the site $\cube$.
	We need to establish this for the map $\ast$, the image of the generator $\product$.
	Diagrammatically, this is equivalent to the commutativity of
	\begin{equation} \label{e:hopf diagonal and the product}
		\begin{tikzcd}
			\product \otimes \chains(\cube^{p+q})^{\otimes 2} \arrow[d] \arrow[r, "\Delta_\M \otimes Sh"] &[20pt]
			\left(\, \ \leftboundary \ \otimes \product + \product \otimes \ \rightboundary \ \, \right) \otimes \chains(\cube^{p})^{\otimes 2} \otimes \chains(\cube^{q})^{\otimes 2} \arrow[d]\\
			\chains(\cube^{p+q}) \arrow[r, "\cong"] &
			\, \chains(\cube^{p}) \otimes \chains(\cube^{q}).
		\end{tikzcd}
	\end{equation}

	Since this commutativity is immediate for $p = 0$ or $q = 0$ and $\chains(\cube^n) \cong \chains(\cube^1)^{\otimes n}$, we only need to verify it for $p = q = 1$.

	Consider $(x_1 \otimes y_1) \otimes (x_2 \otimes y_2) \in \chains(\cube^1)^{\otimes 2} \otimes \chains(\cube^1)^{\otimes 2}$.
	We have that
	\[
	\big((\id \otimes \varepsilon) \otimes \ast \ + \ \ast \otimes (\varepsilon \otimes \Delta)\big) \ (-1)^{\bars{y_1} \bars{x_2}} \ (x_1 \otimes x_2) \otimes (y_1 \otimes y_2)
	\]
	is equal to
	\begin{align*}
		& (-1)^{\bars{y_1} \bars{x_2} + \bars{x_1} + \bars{x_2} + \bars{y_1}} \ x_1 \cdot \varepsilon(x_2) \otimes y_1 \ast y_2 \\ + \
		& (-1)^{\bars{y_1} \bars{x_2} + \bars{x_1}} \ x_1 \ast x_2 \otimes \varepsilon(y_1) \cdot y_2.
	\end{align*}
	The first summand is non-zero only if $\bars{x_2} = \bars{y_1} = \bars{y_2} = 0$, whereas the second is non-zero only if $\bars{x_1} = \bars{x_2} = \bars{y_1} = 0$, so the above is also equal to
	\begin{equation} \label{e:join is monoidal 1}
		(-1)^{\bars{x_1}} \ x_1 \cdot \varepsilon(x_2) \otimes y_1 \ast y_2 \ + \
		x_1 \ast x_2 \otimes \varepsilon(y_1) \ast y_2.
	\end{equation}
	On the other hand,
	\begin{align*}
		(x_1 \otimes y_1) \ast (x_2 \otimes y_2) \ & =\
		(-1)^{\bars{x_1} + \bars{y_1}} \ (x_1 \ast x_2) \otimes \varepsilon(y_1) \cdot y_2 \\ & +\
		(-1)^{\bars{x_1} + \bars{y_1}} \ x_1 \cdot \varepsilon(x_2) \otimes (y_1 \ast y_2) \\ \ & =\
		(x_1 \ast x_2) \otimes \varepsilon(y_1) \cdot y_2 \\ & +\
		(-1)^{\bars{x_1}} \ x_1 \cdot \varepsilon(x_2) \otimes (y_1 \ast y_2),
	\end{align*}
	which is equal to \eqref{e:join is monoidal 1} as claimed.
\end{proof}

%	In diagrammatic terms,
%	\[
%	\begin{tikzcd}
	%	\coproduct \otimes \chains(\cube^{p+q}) \arrow[r, "\Delta_\M \otimes Sh"] \arrow[d] &[20pt]
	%	\left( \ \coproduct \otimes \coproduct \ \right) \otimes
	%	\chains(\cube^{p}) \otimes \chains(\cube^{q}) \arrow[d] \\
	%	\chains(\cube^{p+q})^{\otimes 2} \arrow[r, "Sh"] &
	%	\chains(\cube^{p})^{\otimes 2} \otimes \chains(\cube^{q})^{\otimes 2}
	%	\end{tikzcd}
%	\]
%	and
%	\[
%	\begin{tikzcd}
	%	\counit \ \otimes \chains(\cube^{p+q}) \arrow[r, "\Delta_\M \otimes Sh"] \arrow[d] &[20pt]
	%	\left( \ \counit \ \otimes \ \counit \ \right) \otimes
	%	\chains(\cube^{p}) \otimes \chains(\cube^{q}) \arrow[d] \\
	%	R \arrow[r, "\cong"] &
	%	R \otimes R
	%	\end{tikzcd}
%	\]
%	commute.

